ConvoKit: A Toolkit for the Analysis of Conversations

This paper describes the design and functionality of ConvoKit, an open-source toolkit for analyzing conversations and the social interactions embedded within. ConvoKit provides an unified framework for representing and manipulating conversational data, as well as a large and diverse collection of conversational datasets. By providing an intuitive interface for exploring and interacting with conversational data, this toolkit lowers the technical barriers for the broad adoption of computational methods for conversational analysis.

==> FIG/table-transformers.tex <==
% !TEX root = ../paper-main.tex

\begin{table}[ht!]
	% \centering
	\begin{tabular}{p{0.04\textwidth}p{0.36\textwidth}}
		\toprule
		Type & \ \ \ Transformers \\
 		\midrule
		{\rotatebox[origin=category]{90}{Preprocessors }} & \parbox[t]{0.36\textwidth}{Text parser \newline Text cleaner \newline Syntactic patterns (TextToArcs) \newline \textit{Merging users / utterances} \newline \textit{Data de-duplication}} \\
		\midrule
		{\rotatebox[origin=category]{90}{Feature extractors \ \ }}  & \parbox[t]{0.36\textwidth}{Politeness strategies \newline Structural features (HyperConvo) \newline Linguistic coordination \newline Speech act tagging~(PromptTypes) \newline Speaker diversity  \\ \textit{Arrival order} \\ \textit{Tree depth} \\ \textit{Sentiment analysis}} \\
		\midrule
		{\rotatebox[origin=category]{90}{Analyzers \ \ \ \ }} & \parbox[t]{0.36\textwidth} {Classifier/Regression \newline Paired prediction \newline Ranker \newline Fighting words \newline Forecaster \newline \textit{Clustering} \newline \textit{Conversational trajectory clustering}} \\
		 \bottomrule
	\end{tabular}
	\caption{A subset of Transformers available in ConvoKit and planned future Transformers (\textit{italicized}), grouped by category.} \ly{condense preprocessing}
	\label{tab:transformer_categories}
\end{table}
